Diffusion Models already have a Semantic Latent Space

Diffusion models achieve outstanding generative performance in various domains. Despite their great success, they lack semantic latent space which is essential for controlling the generative process. To address the problem, we propose asymmetric reverse process (Asyrp) which discovers the semantic latent space in frozen pretrained diffusion models. Our semantic latent space, named h-space, has nice properties for accommodating semantic image manipulation: homogeneity, linearity, robustness, and consistency across timesteps. In addition, we introduce a principled design of the generative process for versatile editing and quality boost ing by quantifiable measures: editing strength of an interval and quality deficiency at a timestep. Our method is applicable to various architectures (DDPM++, iD- DPM, and ADM) and datasets (CelebA-HQ, AFHQ-dog, LSUN-church, LSUN- bedroom, and METFACES). Project page: https://kwonminki.github.io/Asyrp/

==> trash_bin.tex <==
% \fref{fig:add_random_noise} shows the result of adding noise $z$ at different spaces, \textit{$\epsilon$-space} and \hidden, for shifting $\epsilont$. In the case of \textit{$\epsilon$-space}, we should notice the assumption of DDPM. That is, when model is trained, all $\epsilon$ are sampled from $\epsilon \sim \mathcal{N}(0,\mathbf{I})$.
% \section{Full editing process and \capacity{}}
% \section{Analysis on time steps for editing process}
% \begin{equation}
%     \begin{aligned}
%         \tedit(y_{\mathrm{source}}, y_{\mathrm{target}}) &= \argmin_{\tedit} (|\lpips(\vx, \mathbf{P}_{\tedit})-0.33\langle y_{\mathrm{source}}, y_{\mathrm{target}} \rangle|), \\
%         \langle y_{\mathrm{source}}, y_{\mathrm{target}} \rangle&=E_{\mtext}(y_{\mathrm{source}})\cdot E_{\mtext}(y_{\mathrm{target}}),
%     \end{aligned}
% \end{equation}
% Since \capacity{} of $\vx_t$ becomes smaller across timesteps, editing in later stage can brings unexpected results because of insufficient capacity. (See \sref{over_boundary} for examples.) Therefore, we restrict the editing interval to $[T, \tedit]$ instead of $[T, 0]$. We observe that small $t_{edit}$ (i.e. longer interval) leads to the larger change in $\vx_0$. The proper $\tedit$ varies across datasets, noise schedules, and target attributes. Because its brute-force tuning is troublesome, we propose a formula for choosing $\tedit$.

% We decide to limit the editing interval to $[T, t_{edit}]$ (not $[T, 0]$) referring to previous works that argue diffusion models learn perceptually rich visual concepts as $t$ is sufficiently large and the interval needs to be properly selected where high-level contexts is generated. (\citet{meng2021sdedit}, \citet{choi2022perception}, \citet{chung2022come})

% We observe that how $t_{edit}$ is determined is a key factor in image editing . Intuitively, if $t_{edit}$ is close to $T$, the editing interval is shortened accordingly and vice versa. Hence, it can be considered as a hyperparameter that influences on degree of editing.
% Inappropriate $t_{edit}$ leads to unintended changes, and we observe $t_{edit}$ has to vary with datasets, noise schedules, and attributes. We propose a formula that can effectively respond to these three variables.
% Therefore we argue that $\epsilont$ is considered as standard Gaussian variable.

% If we add $z \sim \mathcal{N}(0,\sigma\mathbf{I})$ to $\epsilont$, $z$ might be able to harm distribution. Hence we conduct experiments two ways, $\tepsilont = \epsilont + z$ and $\tepsilont = (\epsilont + z) / \sqrt{1^2 + \sigma^2}$. However even if we kept variance of $\epsilont$, the result showed exactly the same pattern as \fref{fig:add_random_noise}.

% Meanwhile, as respect to \hidden \, we observed that considering mean or variance of \hidden \ has a rather bad effect; that leads to lose original information, identification. 

% And when we use original DDIM reverse process, not \ours, \fref{fig:add_random_noise}-(a) shows barely changed image even if we opt to use $z \sim \mathcal{N}(0,\mathbf{I})$.

% Recently, diffusion-based generative models have emerged in the spotlight for image synthetics.(\cite{ho2020denoising}) They have shown better or competitive performance compared to other generative models, e.g., generative adversarial networks (GANs), in the aspect of diversity, mode coverage and fidelity \needcite{}. They are also rapidly finding usage in other domains and tasks such as video (\cite{ho2022video}), audio (\cite{kong2020diffwave}), text generation (\cite{austin2021structured}), protein structure and sequence generation (\cite{anand2022protein}), reinforcement learning (\cite{janner2022planning}), and segmentation (\cite{wang2022semantic}). Especially, they have shown the possibility of real-image editing because the nearly perfect inversion of the image is effortless. (\cite{song2020denoising})
% Note that it is different from the diffused noise-space of latent variables and the use of the latent space conducts on fixed pre-trained model. 
% \fref{fig:cdmvsclipvsours} illustrates remarkable advantages of our method over the existing methods; using vanilla diffusion models, even not requiring additional heavy training or computation as in classifier guidance model and not fine-tuning the whole diffusion model as in DiffusionCLIP. As defined above, demonstrated semantic latent space, named \hidden{}, can effectively change the images with intuitive control.

% However, the all prior works require new learning with the appropriate architecture and fail to find the semantic latent space of vanilla diffusion models.
% However, there is no \textit{semantic latent space} clarified in diffusion models, unlike other generative models.
% We define \textit{semantic latent space} as following descriptions: changes in the space should bring meaningful changes in image space e.g., facial attributes, hairstyle, and age. And the space should be intuitively controllable. 
% For example, linear property can play a role in the controllability. Under the property, i) interpolation or extrapolation of a change on latent space causes a corresponding semantic change in an image ii) addition of changes on latent space causes addition of corresponding changes in an image.


% Other generative models, e.g., GANs and variational autoencoders (VAE), have controllability affected by latent space. Conversely, diffusion models lack \textit{semantic latent space} although they can be considered as latent variable models. \cite{kim2021diffusionclip} experimentally shows the less-semantic of the diffused latent variable by directly optimizing latent variable. It prevents diffusion models from guaranteeing controllability while GANs have shown tremendous performance in conditional generation and image editing by exploiting the ability of latent space.

%Unfortunately, existing methods can rarely handle Diffusion models by the semantic latent space. (\needcite{DiffusionCLIP} shows that.) It prevents diffusion models from guaranteeing controllability while GANs have shown tremendous performance in conditional generation and image editing by exploiting the ability of latent space.


% As a consequence, diffusion models attempt to guarantee the controllability by two main methods. The first one is indirect guidance on vanilla diffusion models e.g., image-space guidance (\cite{choi2021ilvr}, \cite{lugmayr2022repaint}, \cite{meng2021sdedit}), classifier guidance (\cite{dhariwal2021diffusion}, \cite{avrahami2022blended}, \cite{liu2021more}), \cite{sehwag2022generating}, and fine-tuning the whole model (DiffusionCLIP).
% However image-space guidance method generates images using conditioned images or strokes, which as a result brings less controllability because of the process of itself. (\fref{compare_sampling}-(b)) Classifier guidance method requires extra classifiers that should robust on noisy images and costs additional computation for sampling with gradients of the classifiers. (\fref{compare_sampling}-(c))
% And DiffusionCLIP requires fine-tuning the whole models even if it does not suffer from these problems. (\fref{compare_sampling}-(d))

% Second, there are attempts to design inductive biased architecture for mounting external latent space.
% \cite{preechakul2022diffusion} adjusts the architecture of diffusion models so as to use a latent space by integrating diffusion models with AutoEncoders. \cite{rombach2022high} and \cite{vahdat2021score} try to integrate latent variable of diffusion models with latent variable of AutoEncoders or VAE.
% However, the all prior works require new learning with the appropriate architecture and fail to find the semantic latent space of vanilla diffusion models.


%\js{Semantic latent space is the essential of generative models. It means the compressed representation of a data, such as features or combinations of the features which are meaningful to human. By analyzing latent representation in the latent space, we can understand patterns or structural similarities between data points. The latent space can be used for interpolation of data and generation of samples.}

%\uh{However, diffusion models의 latent space는 GAN과 달리 semantic meaning이 없다. It prevents the diffusion models from 확보하기ing controllability while GANs는 conditional generation and editing 잘된다. 그래서 controllability를 간접적인 guide 등으로 확보한다~ 다음문단 붙이기}
 %But unfortunately, semantic latent space is hardly found in Diffusion models although they can be considered as latent variable models. It leads the most of recent works in Diffusion models to edit semantic information of images not by directly controlling the latent space but exploiting indirect types of sampling methods, e.g. stroke guided \needcite{SDEdit}, classifier guidance \needcite{BeatGANs, Blended}, masked area generating \needcite{Blended, Repaint}, image editing with fine-tuning of the whole model \needcite{DiffusionCLIP}, etc.

%\uh{진정한 semantic latent space가 필요하다는 단락으로 무게를 주세요. 이것도 figure1처럼 시각적 비교가 있으면 이해가 빠를것같은데 가능할까요?} 

%\uh{GAN이 semantic의 중요함을 보인건 아니고 중요함은 원래 거기 있던거예요. 여기서 GAN의 inversion구림을 깔 필요는 없습니다. GAN은 비교대상으로만 언급하는 형태로 윗윗문단에 합쳤습니다.} %On the other hands, GANs have shown the importance of semantic latent space. \needcite{StyleCLIP, ADA, 등등} show good performance in image editing as well as image generation using semantic latent space. However, it is the weakness of GANs that inaccurate inversion methods \needcite{} degrade overall performance in real image editing .

%\uh{우리가 발견한 semantic latent로 뭘 할수있다는 문단}
%After all, we demonstrate that the vanilla diffusion models already have a semantic latent embedding space other than the diffused noise-space when paired with our BM-sampling method even though using fixed pre-trained model.
% After all, we propose third one. We demonstrate that the vanilla diffusion models already have a \textit{semantic latent space} when paired with our Asymmetric Reverse Process via h-space (\ours). Note that it is different from the diffused noise-space of latent variables and the use of the latent space conducts on fixed pre-trained model. 
% \fref{fig:cdmvsclipvsours} illustrates remarkable advantages of our method over the existing methods; using vanilla diffusion models, even not requiring additional heavy training or computation as in classifier guidance model and not fine-tuning the whole diffusion model as in DiffusionCLIP. As defined above, demonstrated semantic latent space, named \textit{h-space}, can effectively change the images with intuitive control.

% Through the paper, we extend the controllability of \hidden{} during a generative process to real-image editing utilizing the nerarly perfect effortless inversion property of DDIM.
%Through the paper, we focus on editing images while a generative process that can be easily extended to real-image editing because of the nearly perfect effortless inversion property of DDIM. 
% As for editing, we present the way to measure how much implicit or explicit information is lost with respect to time steps. And then we provide a principled way of editing according to the measurement; which is time-dependent (actually, noise-level-dependent). Furthermore, the analysis on the time-dependent information provides a way to further improve the quality of DDIM from the viewpoint of editing. 

%우리가 제시한 time step 대한 anlaysis를 바탕으로 해야지만, h-space상에서 intuitivley control할 수 있는 좋은 특성들(예를 들어 linear property) 을 사용할 수있고, 이를 experimental하게 보인다. 우리는 또한 h-space 상에서의 manipulation이 sample, 더 나아가서 time steps 에 영향을 적게 받음을 분석하였다.

% Applying the analysis on the time step, we show that linear property holds for \hidden{}, which enables intuitive control such as gradual manipulation by interpolation and extrapolation of the semantic latent embeddings even to the unseen intensity and directions (\fref{fig:cdmvsclipvsours} right). We also show \hidden{} is less sensitive to samples and even time steps.

% Experimentally, we show \textit{h-space} has linear property which means linear interpolation and extrapolation of the semantic latent embeddings lead to gradual changes even to the unseen intensity and directions (\fref{fig:cdmvsclipvsours} right). And we analyze properties of \textit{h-space} concluding it is less influenced by samples and even time steps.

% In \sref{sec:main}, we introduce \ours, a new sampling process, which is essential for \textit{h-sapce} and deals with how one can find meaningful directions. Our method achieves cost effective, intuitively controllable, comprehensive and extensive editing. In \sref{noise_level}, we propose strategies to figure out which information diffusion model has at each noise-levels. It brings several beneficial approaches i.e., finding efficient noise levels for image editing, enhancing the image quality of DDIM process, and a formula that enables any length of inference. Results on various architectures and datasets are described in \sref{various_dataset}. And finally, we analyze \hidden \ in \sref{analysis}.

%Additionally, BM-sampling includes noise injection scheme that enhance the image quality of DDIM process which can be used alone. Results on various architectures and datasets are described in \sref{analysis} and \sref{experiment}. And finally, we analysis \textit{h-space} in \sref{analysis}.

%Through the paper, we propose to edit an image with pre-trained vanilla diffusion model using \textit{h-space}.
%With the nearly perfect inversion, our method achieves cost effective, intuitively controllable, comprehensive and extensive editing.
%In \sref{sec:main}, we introduce BM-sampling  which is essential for h-space and deal with how we can find meaningful direction in h-space. In \sref{noise_level}, We propose strategies to find efficient noise levels during sampling process for image editing and conduct experiments to support it. Additionally, BM-sampling includes noise injection scheme that enhance the image quality of DDIM process which can be used alone. Results on various architectures and datasets are described in \sref{analysis} and \sref{experiment}. And finally, we analysis \textit{h-space} in \sref{analysis}.
%In this paper, 우리는 \sref{sec:main} 우선 BM-sampling which is essential for latent space 과 h-space 에 대해 소개한 뒤, h-space에서 의미있는 변화를 만들어낸 방법에 대해서 다룬다. \sref{noise_level}에서 diffusion models에서의 editing을 위한 noise level에 대한 분석과 해결방법을 제안한다.  \sref{analysis}와 \sref{experiment}에서 various 아키텍처와 데이터셋을 통해 h-space의 특성과 그 결과를 보인다. Furthermore, the embedding can be used to classify the attributes of the generated images (\sref{} 실험 section).

% We successfully impose latent space, which is largely employed in GANs, on the generative ability of diffusion models having property of effortless inversion.

%\uh{윗문단에 합체시키기} This paper shows that image editing or conditional sampling is possible with fixed pre-trained diffusion models through semantic latent space; we called h-space.
% As shown in \fref{fig:cdmvsclipvsours}, our work enables image editing   by leveraging the capability of latent space that can be controlled by direction, linear interpolation and extrapolation, 


%The latent space exists in U-Net based models which is generally used in diffusion models and has applicability in various datasets. \uh{이건 다른방법대비장점에 가까운지 semantic에 가까운지 애매하군요. 전자로 승화시킬 수 있으면 좋습니다.}

%\uh{intro가 장황하지 않은데 이런 나열은 여기보다 conclusion으로 옮기면 어떨까요? 이 자리에는 실험결과요약이나 section 구성이 들어가면 좋겠습니다.}
%Our contribution is as follows. 1. To the best of our knowledge, we are the first to introduce the discovery of the semantic latent space of the diffusion model. 2. We propose an BM-sampling method that is essential for the latent space. 3. We propose strategies to find efficient noise levels during sampling process for image editing and conduct experiments to support it. 4. We show various properties of h-space through experiments.
% With \eref{eq:bmsampling}, $\Delta \epsilon^{(t)}$ can be considered as a direction of latent variables. However, as shown \fref{fig:ablation}, this $\epsilon$-space can not be considered as \textit{semantic latent space}. We can get a direction of one single image by directly optimizing $\Delta \epsilon^{(t)}$ but this direction shows less changes and can not be adapted to other images, while $\Delta h$ can. 
% We use $\lambda_2=3$ for all datasets and $\lambda_1=0.8$ for CelebA and LSUN-church, $\lambda_1=1.5$ for LSUN-bedroom, AFHQ-v2 and Metfaces. Note that when we train $f_{df}$ on unseen domain, we fine-tune $\lambda_1$ for each attribute. (See \aref{Appendix_train_detail})
% We select $S=40$ for training $f_{df}$ and $\hat{S}=1000$ for inference. We train $f_{df}$ for 1 epoch using 1000 real images with batch size 16. We figure out that training with \textit{random sampling process} is possible and it shows an advantage on unseen domain and specific attributes which are unnecessary to maintain original appearance. (See \aref{Appendix_train_randomnoise} for details.) Training $f_{df}$ takes about 20 minutes with three RTX3090s.
% All figures are not used for the training unless mentioned specifically.
% 우리는 40step으로 델타블록을 학습하였으며 sampling은 1000step을 사용하였다.
% 학습 이미지는 1000장을 사용하였으며 out of domain과 AFHQ의 경우 random noise 1000장을 사용하여 학습하였다. 이에 대한 자세한 정보는 \aref{Appendix_train_randomnoise}에 있다.
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
%And we failed to learn the network for $\Delta \epsilon^{(t)}$. 

%We have shown that we can edit each sample effectively with $f_{df}$, and 
%but that does not prove that \textit{h-space} is a general space. 
% Therefore, we opt to use a mean direction $\Delta h_t^{mean}$, the average $\Delta h_t$ of 20 images. Figs show that the mean direction is fitted on any image that means less affected by samples.
% \sref{Appendix_global} show that the mean direction works and is insensitive over samples.
% Furthermore, we broadcast $\Delta h^{global}$, as described in \sref{section_global}, to every editing time steps and then we indicate global direction $\Delta h^{global}$ shows a similar effect as mean direction. 

% Furthermore, we get a global direction, $\Delta h^{global}$, by broadcasting $\Delta h_{t}$ over time steps. Experimentally, $\Delta h^{global}$ shows similar editing results compared to $\Delta h^{mean}$.
% Hence, we postulate that \hidden{} can be shared throughout time steps and less influenced by them.It gives us not only the virtue of simplicity but also the benefit with an aspect of computational cost by global direction. 
%We hypothesized all directions and \textit{h-space} are similar whether what time steps.
%We investigate it by broadcasting a $\Delta h_t$ for all editing process. \fref{fig:global}-(right) shows that when we broadcast direction of any time steps, the results do not have significant differ.
%Even if we use global direction for all editing process, it works well like mean direction. 
%But we observe that result of broadcasting $\Delta h_t$ could be slightly different on the unseen domains. (See \aref{Appendix_global}.) 
%Even on unseen domain, conducting with the global direction is pretty alike to the mean direction and that supports \textit{h-space} is shared throughout time steps.

% DeltaBlock을 사용해서 방향을 찾기 위해서는 모든 샘플들을 다 하나씩 네트워크를 통과시켜서 direction을 찾아야 한다. 이 때 여러개의 delta h를 평균내도 어느정도 비슷한 결과를 얻을 수 있다. 피규어는 우린 총 8장의 이미지들을 통해 평균낸 delta h로도 잘 웃는 모습을 보여준다. 이를 통해 h-space가 샘플마다 각각의 space를 가진 것이 아닌 global한 space임을 간접적으로 알 수 있다. 따라서 global directions 만 알고 있다면 DeltaBlock 조차 없어도 BM-sampling이 가능하다.

% \subsection{global of global directions}
% Note that DeltaBlock에 input으로 timestep t가 들어가며, 이에 따라 delta h는 t에 디펜던트하다. 하지만 모든 timestep에 대해 direction을 평균내서 적용해도 잘 웃는다.  즉, delta h는 동일한 attribute에 대해서는 samples와 timestep과 크게 상관 없이 비슷하단 것을 알 수 있다. 

% We focused on not only time steps as a different role but also accelerating. 
% Thanks to accelerated generating process of DDIM, we are not forced to sample T steps as training $f_{df}(h,t) = \Delta h_t$. As in DDIM, the forward process can be defined on a subset $x_{\tau_1},...,{x_{\tau_S}}$ where $S$ is  length of sub-sequence which can be an arbitrary number. All the figure we present is from $f_{df}$ trained on the subset.

scaling dh
% Even if $f_{df}$ is trained on the subset, the reverse process is not forced to sample on it. Any subset with length of $\hat{S}$, not included in the subset which we use to train the network, can be applicable by scaling $\Delta h_{t}$.
% We hypothesize that if the total amount of $\Delta h_{t}$ is equal, the similar alteration occurs. 
% Since $\Delta h_{t}$ means the amount of changes corresponding to the step interval of the training subset, we should scale $\Delta h_{t}$ corresponding to the step interval of the subset of generative process by $\Delta \hat{h}_t=(S / \hat{S}) \Delta h_{t}$.
% To this end, with $f_{df}$ trained on any subset, the generative process is enabled with the any other subset. See more details in \aref{Appendix_scaling}


%         \Function{Editing}{$x_{0}$,$\epsilon_{\theta}$,$\{\lambda_{i}\}^{M}_{i=1}$, $S_{gen}$,$*$}
%     \begin{algorithmic}[1]
%         \State Define $\{\tau_{s}\}^{S_{for}}_{s=1}$ s.t $\tau_{1}=0$,$\tau_{S_{for}}=T$
%         \State \slash\slash step 0: semantic encoding
%         \For{$s=1,2,...,S_{for}-1$}
%             \State  $\epsilon \xleftarrow{} \epsilon_{\theta}(x_{\tau_{s}},\tau_{s})$
%             \State  $x_{\tau_{s+1}}=\sqrt{\alpha_{\tau_{s}}}x_{\tau_{s}}+\sqrt{1-\alpha_{\tau_{s}}}\epsilon$
%         \EndFor
%             \State Define $\{\hat{\tau}_{s}\}^{S_{gen}}_{s=1}$ s.t ${\hat{\tau}_{1}}=0$,$\hat{\tau}_{S_{edit}}=t_{edit}$,${\hat{\tau}_{S_{noise}}}=t_{noise}$, and ${\hat{\tau}_{S_{gen}}}=T$
%             \State \slash\slash step 1: manipulation
%             \State  $\hat{x}_{S_{gen}}=x_{S_{for}}$
%         \For{$s=S_{gen},S_{gen}-1,...,2$}
%             \If{${s \ge S_{edit}}$}
%                 \State  $\Delta{h}_{\hat{\tau}_{s}}=\frac{S_{for}}{S_{gen}}(\sum_{i=1}^{M}\lambda_{i}f^{i}_{df}(\hat{x}_{\hat{\tau}_{s}}))$
%                 \State $\hat{\epsilon}=\epsilon_{\theta}(\hat{x}_{\hat{\tau}_{s}}|\Delta{h}_{\hat{\tau}_{s}})$
%                 \State $\epsilon=\epsilon_{\theta}(\hat{x}_{\hat{\tau}_{s}})$
%                 \State $\sigma_{t}=0$
%             \Else\If{$s \ge S_{noise}$}
%                 \State $\hat{\epsilon}=\epsilon=\epsilon_{\theta}(\hat{x}_{\hat{\tau}_{s}})$
%                 \State  $\sigma_{\hat{\tau}_{s}}=0$
%             \Else
%                 \State $\hat{\epsilon}=\epsilon=\epsilon_{\theta}(\hat{x}_{\hat{\tau}_{s}})$
%                 \State  $\sigma_{\hat{\tau}_{s}}=\sqrt{\left(1-\alpha_{\hat{\tau}_{s}-1}\right) /\left(1-\alpha_{\hat{\tau}_{s}}\right)} \sqrt{1-\alpha_{\hat{\tau}_{s}} / \alpha_{\hat{\tau}_{s}-1}}$
%             \EndIf
%         \EndIf
%             \State $z\sim N(0,1)$
%             \State $\hat{x}_{\hat{\tau}_{s-1}}=\sqrt{\alpha_{\hat{\tau}_{s-1}}}(\frac{\hat{x}_{\hat{\tau}_{s}}-\sqrt{1-\alpha_{\hat{\tau}_{s}}}\hat{\epsilon}}{\sqrt{\alpha_{\hat{\tau}_{s}}}})+\sqrt{1-\alpha_{\hat{\tau}_{s-1}}-\sigma^{2}_{\hat{\tau}_{s}}}\epsilon+\sigma_{\hat{\tau}_{s}}z$
%         \EndFor
%         \State \Return{$\hat{x}_{0}$ (manipulated image)}
    
%     \end{algorithmic}
% \end{algorithm}
% One straightforward approach is to compute the difference between $\vx_t$ and the original image $\vx$. It provides some understanding in the generative process but it hardly evolves during the first 80\% of progress \citep{choi2022perception}.

%\fref{fig:comparing_1000_40} shows that similar results are produced in different inference steps. This result shows that our proposed scaling works very well i.e., the difference is only the quality due to fast sampling of DDIM, and the degree of change in attributes is the same. We assume that less influenced by time steps is the main cause of it. A similar change can be guaranteed if the total amount is preserved accordingly. This gives a very great advantage of being able to obtain free steps and quality despite fast training. Furthermore, it is possible after checking the result of editing by fast sampling with a small step, then the finally determined sample can be generated with high quality. In the case of our experiment, it took about 1.5 seconds to sample at 40 steps, and it took about 40 seconds to sample at 1000 steps.

h-space
In addition, when we set $\depsilon$ as random noise, we observe that directly adding random noise to $\epsilon$-space cannot bring semantic changes but only noisy and meaningless results and it is sensitive to added magnitude of $\depsilon$. (See \fref{fig:add_random_noise}(c).)

%The loss induces a difference between direction from  source image to a target image and direction from a reference text to a target text on CLIP embedding space. 
%\uh{$\vx_T$나 $\depsilon$ 구할때는 loss를 식으로 정의하지 않고 말로만 설명하고 넘어가는게 독자입장에서 이해가 불완전할까 염려됩니다.}
%\begin{equation}
%\mathcal{L}_{\text {direction }}\left(\boldsymbol{x}^{\text {gen }}, y^{\mathrm{tar}} ; \boldsymbol{x}^{\text {ref }}, y^{\text {ref }}\right):=1-\frac{\langle\Delta I, \Delta T\rangle}{\|\Delta I\|\|\Delta T\|}, 
%\end{equation}
%where $ \Delta T=E_{T}\left(y^{\mathrm{tar}}\right)-E_{T}\left(y^{\mathrm{ref}}\right), \Delta I=E_{I}\left(\boldsymbol{x}^{\mathrm{gen}}\right)-E_{I}\left(\boldsymbol{x}^{\mathrm{ref}}\right)$.
%$E_{I}$ and $E_{T}$ are image and text encoders of CLIP, respectively. 
h vs e
We find this feature space resembles the editing property of the latent space of GANs when coupled with \ours{}. $\depsilon$ for an image does not result in the same effect on other images (\fref{fig:ablation}(b)). Furthermore, \fref{fig:add_random_noise}(c) shows that $\vx_0$ easily degenerates with small changes of $\depsilon$. \fref{fig:add_random_noise}(e) shows that adding random $\deltah$ results in plausible images while the adding $\depsilon$ easily degenerate. \aref{Appendix_finding} explores inferior alternative choices.


\subsection{Flexibility of Train/Test Steps and Scaling $\Delta h_{t}$}
\label{step_scaling}

DDIM accelerates generating process by defining forward processes with lengths smaller than $T$. The forward process can be defined on a subset $x_{\tau_1},...,{x_{\tau_S}}$ where $\tau$ is a sub-sequence of $[1,...,T]$ and $S$ is an arbitrary length of the sub-sequence. All the figure we present is from $f_{df}$ trained on a subset where $S<T$.

We note that the reverse process of \ours{} is not forced to sample $S$ steps. By simply scaling $\Delta h$, any subset with a length $\hat{S} < T$ can be applied for sampling. We hypothesize that if the sum of $\Delta h$ along time steps preserves, \ours{} can achieve a similar editing results on user defined subsets $x_{\hat{\tau}_{1}},...,x_{\hat{\tau}_{\hat{S}}}$. Since $\Delta h_{\tau}$ means the amount of changes corresponding to the step interval of the training subset, we scale $\Delta h_{\hat{\tau}}$ by $\Delta h_{\hat{\tau}} = (S / \hat{S}) \Delta h_{\tau}$ for the preservation. See more details in \aref{Appendix_scaling}


\section{Abstract}
%Controllability of generative models are so desired that until now diffusion models have used image-guidance or classifier guidance sampling for manipulation.
%Consequently, previous works tried to guarantee the controllability with the aid of indirect methods, e.g., image guidance or classifier guidance.
% What are the claimed contributions of the paper? : Firstly find out the semantic latent space of vanilla diffusion models.
%To address the problem, we propose a new way of the semantic latent space manipulation with our Asymmetric Reverse Process(ARP). 
% To address the problem, we propose \textbf{asy}mmetric \textbf{r}everse \textbf{p}rocess (\ours{}) which enables manipulation in the semantic latent space.
% \ours{} edits a final result by asymmetrically manipulating only a $predicted \ x_0$ on \hidden{} apart from a $direction \ pointing$ to the next step during the reverse process.
To the best of our knowledge, we first discover the semantic latent space of vanilla diffusion models and conduct real image editing in the space, \hidden{}, utilizing the nearly perfect inversion property of DDIM.


\section{Intro}

% \mingi{샘플링 중간의 latent variables를 교체한다} \js{derive a sample to share desired semantics by matching each image-level variable with a reference image or stroke.}
the conditional reverse process is a completely new concept with a separate image encoder \textit{outside} the diffusion process.
% In this paper, we demonstrate that the vanilla diffusion models already have a \textit{semantic} latent space when paired with our \textbf{asy}mmetric \textbf{r}everse \textbf{p}rocess (\ours{}).
% The semantic latent space found in our method has necessary properties for manipulation: linearity and robustness.
% In the semantic latent space found by our method, the same shift leads to the same semantic changes in the different images as in the traditional non-diffusion embedding spaces. Furthermore, the magnitude of the latent shift controls the degree of semantic changes even to the \textit{unseen} negative extent.
Besides, combination of different latent shifts produces the combined semantic changes in the images, e.g., smiling young face. Surprisingly, the semantic latent space of different timesteps are similar, i.e.,
% Our contributions are the followings.  Our semantic latent space has nice properties for practical editing applications supported by detailed analyses.


% In addition, we design a principled practice on the generative process based on a measure for its \capacity{}. i) The semantic latent editing should be applied before the original image becomes predictable from the reverse-diffused image. ii) Adding stochastic noise at the end of the generative process boosts the quality of the resulting image.

% \ours{} has the following advantages over the existing approaches. It discovers the semantic latent space of a \textit{frozen} vanilla diffusion model, i.e., it does not require additional training of the pretrained diffusion model or a classifier for guidance. It handles various attribute manipulations with a single pretrained diffusion model. It allows intuitive linear control of the attributes. It is generally applicable to various architectures (DDPM++, iDDPM, and ADM) and datasets (CelebA, AFHQ-dog, LSUN-church, LSUN-bedroom, and \textsc{MetFaces}). 
% \mingi{It has practical and convenient properties and we provide a broad analysis of the properties on the discovered semantic latent space.}
% \js{In the experiments, we provide broad analyses of the discovered semantic latent space which is essential to enable successive control of the reverse process.}

\section{clip}

% 써놓으신 paraphrasing은 표절로 여깁니다. CLIP is proposed to make an embedding latent space shared by visual representations and natural language.In CLIP, a text encoder $E_{T}$ and an image encoder $E_{I}$ are learned to match the latent of an image and the corresponding latent of a text. \citep{gal2021stylegan} designs the local directional loss for image manipulation avoiding mode-collapse. The loss induces a distance between direction from a source image to a target image and direction from a reference text to a target text. 
% The loss induces a distance between direction from a source image to a target image and direction from a reference text to a target text. 
% For example, in the case of manipulating facial attribute \textit{smiling}, `face' is a reference text and `smiling face' is a target text. 
% In this papar, we use an abbreviation for each text prompt (e.g. `face' $\xrightarrow{}$  `smiling face' to `smiling').
%In this paper, we use alterable succinct word rather than refer to each text prompt (e.g. we replace 'face' and 'smiling face' to 'smiling').

\section{sec3}

% First, our sampling method is explained and introduction to h-space follows. Lastly, putting these together, we show how semantic directions can be found on h-space. 
% We abbreviate \eref{ddim_reverse} as follow:

\section{problem}

% \footnote{It is demonstrated in their appendix D.5.}).
% However, as experimented in DiffusionCLIP \needcite{diffusionclip}, directly optimizing $x_T$ to synthesize desired attributes using CLIP loss is too challenging to achieve high-quality results and correct manipulation.

\section{asyrp}

% \subsection{BM-Sampling}
% Diffusion models are latent variable model. Continuous diffused noise-spaces can be regarded as latent variables for all time steps. We postulate that shifted marginal distributions, latent variables, modify $p_{\theta}\left(\mathbf{x}_{0: T}\right)$. However, shifted $\epsilont(x_t)$ is offset by the reverse process and does not make shifted latent variables which means there is no significant change in $p_{\theta}\left(\mathbf{x}_{0: T}\right)$. 
%We aim for real image editing thanks to the effortless inversion property of the diffusion model, especially DDIM. \fref{fig:Binder3}-(a) shows nearly perfect inversion property of DDIM.
%To this end, 
% we modify \eref{sampling_eq} to $x_{t-1} = \sqrt{\alpha_{t-1}}\ \Pt(\epsilont(x_t)+z) + \Dt(\epsilont(x_t)+z)$ using random noise $z$ but simply adding noise to $\epsilon_{\theta}$ both on $\Pt$ and $\Dt$does not make any visible changes compared to reconstructions of original sampling process. We prove it not only experimentally(\fref{fig:Binder3}(b)) but also mathematically(See \aref{Appendix_proof}).

% We propose new sampling method for modifying latent variables by adding noise on only $\Pt$.
% Since it is intuitively obvious that adding noise on only $\Pt$ shifts predicted $x_{0}$ and brings modification in results of reconstruction, we change the sampling process with
% $x_{t-1}=\sqrt{\alpha_{t-1}}\ \Pt(\epsilont(x_t)+z) + \Dt(\epsilont(x_t))$. 

% \boldsymbol{x}^{gen}_t = \Pt(\tepsilont(\vx_t)+\depsilon)$ and $\boldsymbol{x}^{ref}_{t}=\Pt(\epsilont(\vx_t))$. We also use L1 reconstruction loss to maintain the content: $\left | \boldsymbol{x}^{gen}_{t} - \boldsymbol{x}^{ref}_{t} \right |$.

% As a consequence, we can find $\depsilon$ which manipulates $\vx_0$ to optimize a directional CLIP loss reflecting text prompts as shown further in \fref{fig:ablation}. 
%We discovery that optimizing $\depsilon$ for each images with the loss leads to corresponding results.
% As a consequence, we observes changes but not semantically meaningful(\fref{fig:Binder3}(c)). Directly adding random noise to $\epsilon$-space cannot bring worthwhile results. 
% Beyond the achievement, we desire the operation to have more straightforward properties as in the latent space of GANs, e.g., linearity between $\depsilon$ and the change in $\vx_0$. 

%In addition, it is not scalable when we want to manipulate multiple images because it requires time-consuming iterative optimization for each image.


\section{h-space}

% To address the problem, we notice on a layer inside of U-Net(Architecture of Diffusion models) which contains implicit information so as to obtain semantically meaningful changes in images.

% In this paper, the layer is named as `\hidden{}' located at the middle of the U-Net which is not influenced by any skip connection and has the smallest dimension.(see Appendix Figure N) \fref{fig:add_random_noise}(d) show the result of adding random noise on \hidden{} in order to change $\Pt$;

% where $\tepsilont(\vx_t|\deltah_t)$ adds $\deltah_t$ to $\vh_t$ at \hidden \, $\Delta h_t=z$ and $\eta=0$. As shown in \fref{fig:add_random_noise}(d), a person in the real image is changed into another person. From the results, the \hidden \ can be considered as a semantic space with \eref{bm-sampling} and we name \eref{bm-sampling} as \textbf{A}symmetric \textbf{r}everse pr\textbf{o}cess via \textbf{h}-sp\textbf{a}ce (\ours{}) which is essential for employing \hidden \ as latent space. Details of above experiments are further described in \aref{Appendix_finding}.


% \subsection{Optimize direction at \hidden}
% \label{others}

% By leveraging the ability of \ours{} which can bring semantic changes, we optimize $\Delta h^{attr}_t$ instead of using $z$ as $\Delta h_t$ so that an image is changed corresponding to specific and desired attributes. For the optimization of $\Delta h^{attr}$, we use local directional CLIP loss (\eref{eq:directional_clip}). 

% Referring to \cite{avrahami2022blended}, we use predicted $x_0$ for the loss. At each sampling step, $\boldsymbol{x}^{gen}_t = \Pt(\tepsilont(x_t|\Delta h_t))$ refers to predicted $x_0$ which is edited by \ours{} (\eref{bm-sampling}). $\boldsymbol{x}^{ref}_{t}=\Pt(\epsilont(x_t))$ refers to predicted $x_0$ from original DDIM sampling without the editing. 

% In addition, we use L1 regularization loss to maintain identity of a real image. Putting this together, total loss function $\mathcal{L}^{(t)}$ is as follows.
% \begin{equation}
% \label{optimloss}
%     \mathcal{L}^{(t)}=
%     \lambda_1 \mathcal{L}_{\text {direction }}\left(\boldsymbol{x}^{gen}_{t}, y^{\mathrm{tar}} ; \boldsymbol{x}^{ref}_{t}, y^{\text {ref }}\right) 
%     + \lambda_2 \left | \boldsymbol{x}^{gen}_{t} - \boldsymbol{x}^{ref}_{t} \right \vert
% \end{equation}

% As shown in \fref{fig:Binder3}-right, we can observe a semantic change according to the desired attribute by optimizing $\Delta h$.

\section{Implicit neural directions}
% $\vx_t^\mathrm{gen}=\Pt(\epsilont(\vx_t|\vf_t))$.
% From \sref{others}, we show that a direction of an attribute for each sample can be found by optimizing $\Delta h_t$. However, these methods is not scalable to the increasing number of samples since the optimization is required for each sample. To address the scalability, we use Direction Finding layers $f_{df}(h_t,t) = \Delta h_t$ which outputs $\Delta h_t$ for specific attribute regardless of samples. It consists of only 2-conv layer(See \aref{Appendix_deltablock} for details). 
% Consequently, $x^{gen}_{t}$ from \eref{eq:lossde} can be redefined as $\Pt(\tepsilont(x_t|f_{df}(h_t,t)))$.

% Advantages of $f_{df}$ are ;1. Optimization for each sample is not required.
% 2. $t$ of $f_{df}$ can be interpolated. Second one is covered in \sref{step_scaling}.
% All figures except \fref{fig:add_random_noise} are obtained applying $\Delta h_t$ from $f_{df}$.
% \subsection{Flexibility of Train/Test Steps and Scaling $\Delta h_{t}$}
% \label{sec:stepscaling}

\section{Editing process}
% In order to determine the length of the early stage, we design a principled manner with quantifiable measure of potential editing strength.

% We compute the perceptual distance between the original image $\vx$ and the predicted original image $\Pt$ by $\lpips(\vx, \Pt)$ at $t$. It indicates the amount of modification we can make in the remaining process $[t-1, 0]$. We refer to this quantity as \capacity{}. Note that we use $\Pt$ instead of $\vx_t$ because $\Pt$ reveals the high-level context hidden in $\vx_t$. Then, the difference between \capacity{} at time $T$ and $t$ becomes potential editing strength of the interval $[T, t]$. Indeed, we observe that editing the longer interval leads to the larger change in $\vx_0$. 

% Despite of robustness of \hidden{}, excessive potential editing strength may bring undesirable artifacts as later stage handles fine details and has little influence to semantics. To avoid brute-force tuning for the strength, we design a formula using \capacity{}. 

% In \fref{fig:lpips}, we empirically find that $\Pt$ is visually close to $\vx$ when $\lpips(\vx, \Pt)=0.33$, i.e., the attributes are roughly determined. 
% Thus, we always use \ours{} until $t$ with $\lpips(\vx, \Pt)=0.33$.
% Thus we set the minimum interval of editing the generative process to be $[T, \tprim]$ where $\tprim = \argmin_{\tprim}|\lpips(\vx_{0}, \mathbf{P}_{\tprim})-0.33|$. 

% It is recently revealed that at each noise level, diffusion models learn different visual concepts (\cite{choi2022perception}). Intuitively, it is crucial to know at which noise level we should apply editing. In this section, we present a new way to measure which and how much information is lost; and introduce a principled way of real image editing incorporating the measurement and \ours{}.
% \subsection{\Capacity{}}
% It is obvious that editing in the early stage takes privilege of sharing rich visual concepts learned by diffusion models.
% We design a quantifiable measure \capacity{} of $\vx_{t}$: how large modification we can make in the process from the intermediate images $\vx_t$ to the resulting image $\vx_0$. It is foundation for the principled practices in choosing intervals for semantic editing and \qualityboosting{}.
% Since \capacity{} of $\vx_t$ becomes smaller across timesteps, editing over the boundary can brings unexpected results because of insufficient capacity.
% \js{In this section, we provide a principled practice on the diffusion timesteps. Based on quantifiable measurement, the practice enables reasonable choice of editing and noise injection period which leads directly to success in editing.}
% Because the generative process in $[T, t]$ is finished at $t$, we seek to measure the amount of changeable attributes in $[t-1, 0]$.
% Recalling that $\Pt$ denotes predicted $\vx_0$ from $\vx_t$, $\vx_t$ inherently carries the forecast with some discrepancy. We propose to measure this discrepancy as $\lpips(\vx, \Pt)$ to estimate the \capacity{} of the generative process in $[t-1, 0]$ where $\lpips$ computes perceptual distance between the arguments \citep{zhang2018unreasonable}.
% Recalling that $\Pt$ denotes predicted $\vx_{0}$ from $\vx_{t}$, $\vx_{t}$ inherently carries the forecast with some discrepancy. We propose to measure this discrepancy as $\lpips(\vx,\Pt)$ to estimate the flexibility where $\lpips$ compute perceptual distance between the arguments \citep{zhang2018unreasonable}.
% \js{However, at the most of timesteps, one can hardly find the noticeable difference between them except for at near the end of sampling.}
% \js{We measure information intrinsic to the latent variable $x_t$ at each time steps. First, as in \cite{choi2022perception}, we measure the difference between the intermediate $x_t$s and the $x_0$ which is the consequence of it. However, at the most of timesteps, one can hardly find the noticeable difference between them except for at near the end of sampling. We propose an alternative which measure the amount of the difference between by LPIPS(\cite{zhang2018unreasonable}) as shown in \fref{fig:lpips}. }

%Note that $\Pt$ is similar to $\vx$ even when $\vx_t$ has severe noise.

% From \fref{fig:lpips}, we can find that $\Pt$ is visually similar to $x_{0}$ even when $x_{t}$ is not recognizable for noise. $\Pt$ can be considered as implicit information which can be obtained at $t$. To measure how much information $\Pt$ contains, we use LPIPS \cite{zhang2018unreasonable} as in \cite{choi2022perception}. The prior analyzes only on diffused noise-space between two different images, not considering the implicit information at $t$. 
%diffusion models by computing LPIPS distance of two different images, $x^1$ and $x^2$ by gradually adding noise. 
% In contrast, we analyze by computing $LPIPS(x_{0}, \Pt)$ and $LPIPS(x_{0}, x_{t})$ which represent how much information with in a sample $x_{0}$ is lost by noise in $\Pt$ and $x_t$ respectively. As shown in \fref{fig:lpips}, we observe $\Pt$ usually preserves more information compared to $x_{t}$.
%Based on the result, it can be concluded that we can measure implicit information which diffusion models actually has at $t$ not from $x_t$ but from $\Pt$. 
% Based on the result, we conclude that it is $\Pt$ not $x_{t}$ where one can measure implicit information of diffusion models at $t$. The amount of implicit information at $t$ can be demonstrated by $LPIPS(x_{0}, \Pt)$. The larger the information is, the smaller the distance gets.
% In other words,
% there exists time interval when diffusion models has sufficient information of $x_{0}$, even if $x_{t}$ is barely distinguishable from noise during the interval.
% In other words, there exists $t$ at which diffusion models has sufficient information of $x_{0}$, even if $x_{t}$ is barely distinguishable because of noise at the same time.

% Contrary to \cite{choi2022perception} which 
% The difference between the intermediate images $\vx_t$ and the resulting image $\vx_0$ is measured by $LPIPS(\vx_t)$}

\section{Implementation details}
For all datasets, we set $\lambda_\mathrm{recon}=3$ and  $\lambda_\mathrm{CLIP}=0.8 $ or $ 1.5$. Note that only on unseen domain, we fine-tune $\lambda_\mathrm{CLIP}$ for each attribute. (See \aref{asec:train_detail} for dataset-architecture pairs in detail.)
Regarding some attributes, we train $\vf_t$ with random generation .(See \aref{Appendix_train_randomnoise} for details.)

\section{Experiments}

%------------원래 내용입니다 위의 문단과 합쳐야함----------------
% From \eref{eq:bmsampling}, we experiments 2 options of $\Delta \epsilon_{t}$ as a direction of latent variable. \fref{fig:optim} shows the necessity of \hidden{}. On $\epsilon$-space, only optimization of $\Delta \epsilon_{t}$ per sample is possible, while it is challenging to adapt the optimized direction to the other samples. 
% Additionally, as mentioned in \todo{reference제대로}, optimizing $\Delta \epsilon_{t}$ is too sensitive to train $\vf_t$ on \textit{$\epsilon$-space}.
%-----------------------------------------
Collectively, the analysis elucidates linearity properties of \hidden{} allowing straightforward editing.


%---------proof of non-changed image------------------%
\begin{equation}
\hat{\vx}_{t-1} = \sqrt{\alpha_{t-1}}\ \Pt(\hepsilont(\vx_t)) + \Dt(\hepsilont(\vx_t))
\end{equation}

\begin{equation}
=\sqrt{\alpha_{t-1}} \left(\frac{\vx_{t} -\sqrt{1-\alpha_{t}}\left( \epsilon_{\theta}^{(t)}\left(\vx_{t}\right)+\Delta \epsilon_{t}\right)}{\sqrt{\alpha_{t}}}\right)+\sqrt{1-\alpha_{t-1}-\sigma_{t}^{2}} \cdot \left(\epsilon_{\theta}^{(t)}\left(\vx_{t}\right) + \Delta \epsilon_{t} \right)
\end{equation}

\begin{equation}
= \sqrt{\alpha_{t-1}}\ \Pt(\epsilont(\vx_t)) + \Dt(\epsilont(\vx_t)) - \frac{\sqrt{\alpha_{t-1}} \sqrt{1-\alpha_{t}}}{\sqrt{\alpha_{t}}} \cdot \Delta \epsilon_{t} + \sqrt{1-\alpha_{t-1}-\sigma_{t}^{2}} \cdot \Delta \epsilon_{t}
\end{equation}

\begin{equation}
= \vx_{t-1} + \left(-\frac{\sqrt{1-\alpha_t}}{\sqrt{1-\beta_t}} + \sqrt{1-\alpha_{t-1}}\right) \cdot \Delta \epsilon_{t}  \quad \because \eta = 0
\end{equation}

\begin{equation}
= \vx_{t-1} + \left(-\frac{\sqrt{1-\alpha_t}}{\sqrt{1-\beta_t}} + \frac{\sqrt{1- \prod_{s=1}^{t-1} \left(1-\beta_s\right) } \sqrt{1-\beta_t}}{\sqrt{1-\beta_t}} \right) \cdot \Delta \epsilon_{t}
\end{equation}

\begin{equation}
= \vx_{t-1} + \left( \frac{\sqrt{1-\alpha_t - \beta_t} - \sqrt{1-\alpha_t}}{\sqrt{1-\beta_t}} \right) \cdot \Delta \epsilon_{t}
\quad \because \alpha_t = \prod_{s=1}^{t} \left(1-\beta_s \right)
\end{equation}

    % (a) shows nearly perfect inversion property of DDIM. We add random noise $z$ for shifting $\epsilont$, yielded from the network. (b) shows when we add $z$ to the original DDIM reverse process, $x_0$ barely differs with (a). The lower left picture shows the difference from (a). If we add $z$ with \ours \ in \textit{$\epsilon$-space}, (c) shows the image changes but is destroyed. Furthermore, as right side graph shows, \textit{$\epsilon$-space} is sensitive to added noise levels. On the contrary, (d) shows the change of a identity when in \hidden \ even if (c) and (d) has similar L1 distances.

    % In this section, we introduce two main properties of \hidden; i) Linearity property ii) Consistency property. 
% Firstly, we show the linear property of \textit{h-space} in \sref{linear_property}. And then we demonstrate \textit{h-space} is less affected by samples and propose the global direction by demonstrating it's not being influenced by time steps in \sref{global_direction}.
% \subsubsection{linear property}
% \label{linear_property}

% \fref{fig:interpolation} shows linearity property of \hidden. 
% %First, interpolation of $\Delta h_t$ on \textit{h-space} is possible. Second, even extrapolation is possible as we adapt negative direction on \textit{h-space}.
% The result shows that interpolation of $\Delta h_t$ on \hidden \ brings gradual changes in images. Adaptation of negative $\Delta h_t$ causes editing results that are contrary to the corresponding attributes(Extrapolation). The interpolation and extrapolation of the sample support linearity property of \hidden.

\section{appendix hspace}
%Meanwhile, additive random noise on \hidden{} leads the other results. It only changes the identity or attributes preserving the quality of resulting images.  

%All the experiments in this section uses \ours{} not DDIM. When DDIM is applied, we could hardly find modification both on \hidden{} and \textit{$\epsilon$-space}. \fref{fig:add_random_noise}-(b) shows the results even when we opt to use .
